Do Large Language Models Speak All Languages Equally? A Comparative Study in Low-Resource Settings

Large language models (LLMs) have garnered significant interest in natural language processing (NLP), particularly their remarkable performance in various downstream tasks in resource-rich languages. Recent studies have highlighted the limitations of LLMs in low-resource languages, primarily focusing on binary classification tasks and giving minimal attention to South Asian languages. These limitations are primarily attributed to constraints such as dataset scarcity, computational costs, and research gaps specific to low-resource languages. To address this gap, we present datasets for sentiment and hate speech tasks by translating from English to Bangla, Hindi, and Urdu, facilitating research in low-resource language processing. Further, we comprehensively examine zero-shot learning using multiple LLMs in English and widely spoken South Asian languages. Our findings indicate that GPT-4 consistently outperforms Llama 2 and Gemini, with English consistently demonstrating superior performance across diverse tasks compared to low-resource languages. Furthermore, our analysis reveals that natural language inference (NLI) exhibits the highest performance among the evaluated tasks, with GPT-4 demonstrating superior capabilities.

==> sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}


In conclusion, our comprehensive analysis sheds light on the pivotal role of large language models (LLMs) in the landscape of natural language processing (NLP), emphasizing both their remarkable performance in resource-rich languages such as English and the pressing need to extend their utility to low-resource language settings. Through our investigation of zero-shot learning with various LLMs, we have demonstrated that while LLMs, notably GPT-4, exhibit commendable capabilities in English, their performance in low-resource languages remains a subject of concern. This study underscores the importance of addressing the dearth of research and evaluation in low-resource language contexts, propelled by constraints including dataset scarcity and computational expenses. Our findings not only highlight the existing gap in linguistic capabilities for low-resource languages but also advocate for concerted efforts to bridge this divide. By focusing on tasks such as natural language inference (NLI) and considering performance across different LLM architectures, our research contributes valuable insights into the potential avenues for enhancing the applicability of LLMs in general-purpose NLP applications. Moving forward, concerted interdisciplinary efforts are warranted to bolster research initiatives aimed at refining LLM performance in low-resource language environments, thus fostering inclusivity and accessibility in the realm of natural language processing.




% In this study, we report our evaluation of different LLMs using zero-shot learning for NLI, sentiment, and hate speech tasks in English, Bangla, Hindi, and Urdu languages. We present a detailed comparison of the performances of LLMs for English and low-resource languages. In addition, we also offer a discussion about the performances of LLMs as well as the performances across different tasks. Our evaluation details indicate that LLMs are showing better performances in English than low-resource languages. The performances of our experiments demonstrate that LLMs deliver superior results for simple linguistic tasks such as NLI. 



==> sections/data.tex <==
%\section{Data}
%\label{Data}

This section discusses the publicly available data for three tasks used in our study. We first discuss the data for the NLI task followed by the sentiment task and conclude with the hate speech task. Although each task has some datasets for all the languages individually, only the dataset of the NLI task has been translated into several languages. To fairly evaluate the generalization of LLMs, the translated version of the datasets is mandatory for other tasks. We provide a detailed description of data distribution in Table \ref{tab:data_distribution}.

\paragraph{NLI Task:}
We used the cross-lingual natural language inference (XNLI) dataset \cite{conneau2018xnli} for the NLI task. 
The dataset extends the Multi-genre NLI dataset incorporating the raw text from the second release of the Open American National Corpus. The XNLI dataset is mainly developed for the English language and translated into 15 different languages including Hindi and Urdu languages using human annotators. Each data consists of a premise and hypothesis with a corresponding label\footnote{The class labels for the XNLI dataset are Contradiction, Entailment, and Neutral.}. During the development of the dataset, three different hypotheses were generated by the annotators based on the labels from each premise. 
We select the test set of English, Hindi, and Urdu languages from the XNLI dataset for our experiments.
For the Bangla language, we used the translated version of XNLI \cite{bhattacharjee2021banglabert}. The dataset is translated using the English to Bangla translator model described in \cite{hasan-etal-2020-low}. 
%Although the dataset is translated from the XNLI dataset, the test set is short of 115 data from the original set. 

\paragraph{Sentiment Task:}

For the sentiment analysis task, we used the official test of SemEval-2017 task 4: Sentiment Analysis in Twitter \cite{SemEval:2017:task4}. 
The raw texts were collected from X (formerly known as Twitter) and manually annotated them. 
Primarily, the annotation was completed in five classes which include Strongly Positive, Positive, Neutral, Negative, and Strongly Negative. Later, the labels were re-mapped into three classes where Strongly Positive was combined with Positive and Strongly Negative with Negative classes. 
The SemEval-2017 task 4 offered only English and Arabic data. In this study, we only incorporate the English data.
We translated the English test set for the Bangla, Hindi, and Urdu languages for evaluating the LLMs for the sentiment task. We used the web version of Google Translator\footnote{\url{https://translate.google.com}} with the use of Deep Translator toolkit\footnote{\url{https://pypi.org/project/deep-translator/}}. The quality of translations is moderate due to the tweet texts. We analyzed the translations and found that most of the hashtags were not translated into the target language. Moreover, Hindi translations were far better than Bangla and Urdu.

\paragraph{Hate Speech Task:}

We used the dataset described in \cite{hateoffensive} for our hate speech task. 
The texts were collected from X (formerly known as Twitter) where the annotations were done manually into three categories that include 'Hate', 'Offensive', and 'Neither'. Each data was annotated by at least three people and the final label was consolidated by the majority. Few of the data were discarded where there was no majority. 
The official dataset consists of a total of $24,802$ samples. We first split the data into train, validation, and test splits by $70\%$, $10\%$, and $20\%$ respectively. We only used the test set in our study and the language of the official dataset is English.
For Bangla, Hindi, and Urdu language datasets, we translated the English test set using Google Translator. We randomly sampled 100 entries from each translated dataset to conduct an analysis on the quality of the translation. Our assessment revealed that while efforts were made, the quality of translation was found to be moderate, indicating room for improvement. Notably, certain elements such as hashtag words remained untranslated, and specific terms like 'hairspray,' 'oz,' numerical values, among others, were not adequately translated into their respective languages. 




% \textcolor{blue}{We sampled 100 entries randomly from each translated dataset to analyze the translation quality. The quality of the translation is not good and the hashtags words were not translated. Moreover, some words such as `hairspray', `oz', numbers, etc. have also not been translated into their respective languages.}

%We also noticed the translation quality is moderate and has similar issues to the translation of sentiment task datasets.


==> sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Recent advances in large language models (LLMs) developed significant interest in natural language processing (NLP) across academia and industry. LLMs are known for their language generation capabilities that are trained on billions or trillions of tokens with billions of trainable parameters. Recently researchers have been evaluating LLMs for various NLP downstream tasks, especially question answering \cite{akter2023depth, tan2023can, zhuang2023toolqa}, reasoning \cite{suzgun2022challenging, miao2023selfcheck}, mathematics \cite{lu2023mathvista, rane2023enhancing}, machine translation \cite{xu2023paradigm, lyu2023new}, etc. 


% Assessing LLMs aids in our comprehension of their advantages and disadvantages \cite{chang2023survey}. LLMs have the capability to deal with a wide range of tasks and languages that enable machines to comprehend and generate human-like text. However, the majority of language models have been developed and fine-tuned mainly for high-resource languages, leaving a notable gap in the linguistic capabilities for low-resource languages.



% \textcolor{blue}{
% LLMs have the capability to deal with a wide range of tasks and languages that enable machines to comprehend and generate human-like text. However, the majority of language models have been developed and fine-tuned mainly for high-resource languages, leaving a notable gap in the linguistic capabilities for low-resource languages. Further, the LLMs have opened up new prospects for addressing the linguistic diversity gap. 
% }

%Hence, recently LLM evaluation tools (i.e. lm-harness \cite{eval-harness}, OpenAI evals\footnote{\url{https://github.com/openai/evals}}, and LLMeBench \cite{dalvi2023llmebench}) as well as prompting techniques (promptsource \cite{bach2022promptsource} and chain-of-thoughts prompting \cite{wei2022chain}) have been explored significantly. LLMs have demonstrated outstanding performances and capabilities for reasoning, basic mathematics, and question-answering tasks. % The considerable performances and capabilities of LLMs are leading researchers to explore more in artificial general intelligence \cite{bubeck2023sparks, goertzel2023generative}. 


%many NLP downstream tasks have not been widely evaluated. Moreover,The lack of utilization of LLMs in low-resource language could be because of multiple reasons such as lack of multi-linguality, cross-lingual limitations, etc. However, the use of LLMs is becoming more popular in low-resource languages such as Bangla and Hindi for downstream NLP tasks such as NLI, sentiment analysis, and hatespeech detection. 

Most of the existing works on the evaluation of LLMs are on resource-rich languages such as English. However, the capabilities and performances of LLMs for low-resource languages for many NLP downstream tasks are not widely evaluated, leaving a notable gap in the linguistic capabilities of low-resource languages. In low-resource languages such as Bangla and Urdu, several researchers are handling the scarcity of datasets and other resources in NLI \cite{bhattacharjee2021banglabert}, Sentiment analysis~\cite{hasan2023zero,sun2023sentiment, koto2024zero, kumar2021sentiment} and Hate speech detection \cite{khan2021hate, santosh2019hate}. However, the amount of work that uses LLMs is still very few, mainly due to a few constraints such as dataset scarcity, computational costs, and research gaps associated with low-resource languages. These constraints of low-resource languages require more attention, alongside a focus on high-resource languages, to enhance the applicability of LLMs to general-purpose NLP applications.


To fill the aforementioned gap, we comprehensively analyze zero-shot learning using various LLMs in English and low-resource languages. The performance of LLMs shows that GPT-4 provides comparatively better results than Llama 2 and Gemini. Moreover, the English language performs better on different tasks than low-resource languages such as Bangla, Hindi, and Urdu. The Key contributions are as follows:

\begin{itemize}
    \setlength\itemsep{0em}
    \item To address the limitation of publicly available datasets for low-resource languages, we present datasets for sentiment and hate speech tasks by translating from English to Bangla, Hindi, and Urdu, thereby facilitating research in low-resource language processing.
    
   
    \item We investigate and analyze the effectiveness of different LLMs across various tasks for both English and low-resource languages such as Bangla, Hindi, and Urdu, which suggest that LLMs perform better when evaluated in the English language. %Furthermore, our analysis suggests that the NLI task yields the best performance over sentiment and hate speech tasks, while GPT-4 demonstrates superior performance.

        \item We apply zero-shot prompting using natural language instructions, which contain a description of the task and expected output, which enables the construction of a context to generate more appropriate output.
        
    % \item We compare the low-resource languages, all tested LLMs perform better when evaluated on the English language across the three tested tasks. Furthermore, our analysis suggests that the NLI task yields the best performance over sentiment and hate speech tasks, while GPT-4 demonstrates superior performance.
    
    
    % \item Investigation of zero-shot learning using different LLMs for different tasks.
    % \item Comparative analysis of different LLMs across different tasks.
    % \item Comprehensive analysis of LLMs performances on English \textit{vs} low-resource languages.
    %\item Comparative analysis among the performances of the tasks.


    
    % \item Finally, the findings of this study suggest that more efforts are required to ensure the effectiveness of LLMs for low-resource language processing.
    
    % \item NLI task yields the best performance over sentiment and hatespeech tasks while GPT-4 demonstrates superior performance
    % \item All the LLMs yield better results in English than in Bangla, Hindi, and Urdu across the tasks.
\end{itemize}

%Our comprehensive experiments yielded the following summary of our findings: 

%\begin{itemize}
%    \setlength\itemsep{0em}
%    \item NLI task yields the best performance over sentiment and hatespeech tasks.
%    \item GPT-4 demonstrates superior performance across the tasks.
%    %\item Gemini shows prominent results in NLI and sentiment tasks while Llama 2 delivers superior performances in the hatespeech task.
%    \item All the LLMs yield better results in English than in Bangla, Hindi, and Urdu across the tasks.
    %\item Gemini delivers good performances in Urdu languages without being trained in Urdu data.
%\end{itemize}

%The rest of the paper is organized as follows: Section \ref{sec:related_work} gives a summary of related studies. Section \ref{sec:background} discusses the LLMs that were utilized and describes their contents. We describe the detailed zero-shot learning prompting and experimental details in Section \ref{sec:methodology}. Our findings are presented and discussed in the \ref{sec:result_discussion} section. Finally, we concluded in Section \ref{sec:conclusion}.

==> sections/llm_background.tex <==
\section{Background of LLMs}
\label{sec:background}
We evaluate the test set using three different LLMs. In this section, we discuss the LLM models used in this study in detail.

\paragraph{Generative Pre-trained Transformer 4 (GPT-4) \cite{openai2023gpt}}
GPT-4 is one of the best-performing LLMs to predict the following document sequence, which OpenAI developed in March 2023. The model is trained on data up to September 2021 that supports multimodality. The model has over a trillion trainable parameters with a context length of $8,192$ and $32,768$ tokens. Furthermore, GPT-4 supports multilinguality with a strong performance in all languages. In our study, we used the context window of 8k tokens, which cost approximately $\$30$ per one million tokens.

\paragraph{Llama 2 \cite{touvron2023llama}}
Llama 2 is one of the largest open-source LLMs released by Meta in 2023. The model has different versions (7B, 13B, and 70B) based on the parameter size of the model. The Llama 2 model has been trained on 2 trillion tokens with a context length of $4,096$. In our study, we used the \textit{70B chat} version of the model, which is available through Huggingface Inference API\footnote{\url{https://huggingface.co/inference-api}}. The model is trained on publicly available text, instruction data, and one million human annotations. Although $90\%$ of the training data belongs to English, it can generate results for 50+ languages. 

\paragraph{Gemini \cite{team2023gemini}}
Gemini is the most recent and one of the best-performing LLMs trained on top of the Transformer decoder along with multi-query attention \cite{shazeer2019fast}. Gemini offers 4 different models based on the parameter size. Although the Nano-1 and Nano-2 versions have 1.8B and 3.25B trainable parameters, the parameter sizes for the Pro and Ultra versions are unknown. The Gemini models support multimodal data and are trained on a wide range of data (image, text, audio, and video) sources. Further, the model is trained on a sequence length of $32,768$ tokens to provide a better context understanding for the long texts. As a result, Gemini models offer a context length of $32,768$ tokens. Moreover, Gemini includes safety settings to prevent generating harmful content such as hate, offensive, derogatory, sexual harassment, etc. In our study, we only used the Pro version\footnote{The Pro version costs approximately $\$10$ per million tokens.} of the Gemini model. Although the model supports 38 languages, including Bangla, English, Arabic, and Hindi, it does not currently support Urdu, one of the low-resource languages we analyse in this study.

==> sections/methodology.tex <==
\section{Methodology}
\label{sec:methodology}

\subsection{Prompt Approach}

The performance of LLMs varies depending on the prompt content. Designing a good prompt is a complex and iterative process that requires substantial effort due to the unknown representation of information within the LLM. 
In this study, we applied zero-shot prompting by using natural language instructions. The instructions contain the task description and expected output, which enables the construction of a context to generate more appropriate output. We keep the same prompt for each task across the LLMs. Further, we added role information into the prompt for the GPT-4 model as GPT-4 can take the role information and perform accordingly. In our initial study, we noticed that the Gemini Pro model blocks most of the contents from sentiment and hate speech tasks to predict the desired output due to harmful content in the dataset. To get the predictions for those harmful content, we additionally provide a safety setting that does not block any harmful content. However, the model still blocks derogatory languages. We provided the details of the prompts and safety settings in Appendix \ref{sec:appendix_a}.

\subsection{Experimental Settings}

\subsubsection{Data}
\input{sections/data}


\subsubsection{Data Pre-processing}
The sentiment and hate speech datasets were mainly collected from X and contain URLs, usernames, hashtags, emoticons, and symbols. We only removed the URLs and usernames from the sentiment and hate speech task datasets. We keep the hashtags, emoticons, and symbols with data to understand how LLMs performed with this mixed information. Moreover, we did not perform any preprocessing steps for the XNLI dataset. 

\subsubsection{Evaluation Metrics}
To evaluate our experiments, we calculated accuracy, precision, recall, and F$_1$ scores for all the tasks. We computed the weighted version of precision and recall and the macro version of F$_1$ score as it considers class imbalance.




==> sections/related_work.tex <==
\section{Related Works}
\label{sec:related_work}

LLMs, are proficient in various NLP tasks and have high generalization across several NLP tasks. Despite the incredible generalization of LLMs, there is significant room for improvement in their performance, particularly in low-resource languages such as Bangla, Hindi, and Urdu. Previous study \cite{robinson2023chatgpt} demonstrates the inability of LLMs such as GPT-4 to perform on low-resource (African) languages as well as on high-resource languages. However, LLMs perform well in languages (European) that use the same script as English~\cite{holmstrom2023bridging}. 

%In addition to having performance problems in low-resource languages, LLMs may raise serious ethical questions. AI safety training and red-teaming are usually used to prevent LLMs from generating harmful content. However, these safety mechanisms do not apply to low-resource language. Thus, people can circumvent GPT-4’s safeguard by translating unsafe English inputs into low-resource languages \cite{yong2023low}. Safety issues with LLMs highlight the significance of the study's need to be conducted in low-resource language and the importance of involving low-resource languages while training multi-lingual LLMs. 

\subsection{LLM for English}
Researchers have developed many resources and benchmarks in the past couple of decades for the English language \cite{wang2018glue, williams2017broad}. Moreover, several widely recognized downstream tasks, including NLI, sentiment analysis, and hate speech detection, have been studied in the English language for a long time. NLI involves determining the logical relationship between pairs of text sequences \cite{conneau2018xnli, kowsher2023contrastive}. LLMs can determine the relationships among text sequences and produce results similar to state-of-the-art techniques \cite{pahwa2023bphigh, gubelmann2023truth}. In contrast, Sentiment analysis aims to understand and extract subjective information from textual data, such as opinions, attitudes, emotions, or feelings expressed by individuals or groups. Using LLMs for sentiment analysis could be a fascinating prospect because we do not have to develop datasets or train models, and it still produces identical results \cite{sun2023sentiment, hasan2023zero}. Additionally, Hate speech detection is a challenging but essential task to identify and mitigate offensive or harmful language in text data. Some of the commonly used techniques for detecting hate speech include machine learning \cite{abro2020automatic, mullah2021advances}, deep learning\cite{badjatiya2017deep,zimmerman2018improving}, transformer-based models\cite{mozafari2020hate,alatawi2021detecting}, and LLMs \cite{hee2024recent,garcia2023leveraging}. 

\subsection{LLM for Low-resource Languages}
NLP research works and applications for several downstream tasks mainly focus on high-resource languages. Unlike the English language, the advancement of NLP tasks for low-resource languages made it challenging due to several factors described by \citet{alam2021review}. However, there have been some improvements in the last couple of years for Bangla sentiment analysis focusing on resource development \cite{hasan2020sentiment, islam2021sentnob, hasan2023blp} that attained attention from many researchers to concentrate on solving this issue. However, researchers are focusing on generalizing NLP tasks across the languages. Some of these applications have many limitations for low-resource languages that must be addressed to develop and deploy more generalized universal NLP applications. Some of the recent works on NLI \cite{pahwa2023bphigh, gubelmann2023truth}, Sentiment Analysis \cite{rathje2023gpt, xing2024designing, zhang2023enhancing, zhang2023instruct}, and Hate Speech Detection \cite{hee2024recent,garcia2023leveraging} that utilize LLM are mainly carried out in English languages. Moreover, these works opened up the prospects of exploring LLMs for downstream tasks of low-resource languages.

%These works suggest the usage of LLMs for sentiment analysis could be a very exciting prospect because we do not have to develop datasets or train models, and it still produces identical results. 

%The ability of LLMs to infer new language that was not used during the training could potentially be more beneficial for low-resource languages where it is challenging to train and deploy models due to the scarcity of quality datasets. However, most of the studies in the domain follow traditional machine learning or transformer-based models \cite{jahan2023systematic, chhabra2023literature, islam2021sentnob, hasan2020sentiment}. 
There are few attempts from researchers across different languages to utilize LLM for low-resource languages. Although the number of works involving LLMs is insignificant, researchers of low-resource languages are leaning towards using LLM in recent times.  Some notable works that utilize LLM are in low-resource languages such as Bengali \cite{liu2023knowdee, hasan2023zero, kabir2023benllmeval}, Urdu\cite{koto2024zero}, and Hindi \cite{kumar2021sentiment, koto2024zero} shows LLMs can achieve similar results to traditional machine learning techniques and transformer-based models. 



Existing multilingual benchmarks such as  BUFFET \cite{asai2023buffet}, XTREME \cite{hu2020xtreme}, and XTREME-R \cite{ruder2021xtreme} do not address all four South Asian low-resource languages we are considering in our study.  Moreover, these benchmarks are limited to binary classification tasks and use few-shot learning and instruction fine-tuning of smaller LLMs (such as mT5, mT0) and ChatGPT. At the same time, we focus on multi-class classification and use recent zero-shot learning with state-of-the-art LLMs (i.e. GPT-4, Llama 2, and Gemini Pro). 

We followed a similar translation approach to INDICXNLI \cite{aggarwal2022indicxnli}, Okapi \cite{lai2023okapi}, and BUFFET for cros-lingual data translation. Verification of translated data by native speakers suggests that translated data is of good quality and empirical evidence of our study suggests English hashtags in translated data do not influence the prediction of LLMs. 

LLMs' Superior performance in English languages are well-known fact in the NLP community, however, Gemini Pro in our study produces better performance in low-resource languages in sentiment tasks.

%The performance of LLMs is balanced for all languages \cite{huang2023not, qin2023cross}, and our study uniquely focuses on comparing resource-rich (English) and low-resource (Bangla, Hindi, and Urdu) languages using state-of-the-art LLMs. 

%We selected Bangla, Hindi, and Urdu because they are the most widely spoken yet low-resource languages of South Asia \footnote{https://simple.wikipedia.org/wiki/Languages_of_South_Asia}. Moreover, the authors of the paper are native speakers of these languages. 

%Low-resource languages in our study refer to their scarcity of datasets and other resources rather than limitations in LLM capabilities. 






For low-resource languages, there are significant research gaps in comparison with English. The literature on low-resource languages mainly focused on traditional deep learning and fine-tuning small language models. At the same time, large-scale development has been imposed for resource-rich languages like English. The works that use LLMs to solve downstream tasks in low-resource language are very limited, and the capabilities of LLMs have not been explored properly. To address these issues in this work, we aim to comprehensively use LLMs across several tasks for several low-resource languages such as Bangla, Urdu, and Hindi. 

%Most of the works in the literature use traditional machine learning or transfer-based models for the analysis of low-resource languages. The works that use LLM to solve NLP tasks in low-resource language are very few and most of the work is limited to some extent. To address these issues in this work we aim to perform a comprehensive use of LLMs across several tasks for several low-resource languages such as Bengali, Urdu, and Hindi.  




%\subsection{NLI Task}
%NLI involves determining the logical relationship between pairs of text sequences \cite{conneau2018xnli, kowsher2023contrastive}. Large Language Models (LLMs) can be used to determine the relationships among text sequences and produce results similar to state-of-the-art techniques.\cite{pahwa2023bphigh, gubelmann2023truth}. There is very little work on NLI in low-resource languages like Bengali\cite{bhattacharjee2021banglabert}, Hindi, and Urdu. Furthermore, there is barely any work on NLI that utilizes Large Language Models (LLMs). However, LLMs could be a potential solution in low-resource languages, because LLMs can be utilized without developing a new dataset or training new models. LLMs' excellent cross-lingual performance makes it more beneficial to perform NLI analysis across many languages \cite{liu2023evaluating}. 


%\subsection{Sentiment Task}
%Sentiment analysis aims to understand and extract subjective information from textual data, such as opinions, attitudes, emotions, or feelings, expressed by individuals or groups. Using Large Language Models (LLMs) for sentiment analysis could be a very exciting prospect because we do not have to develop datasets or train models, and it still produces identical results \cite{sun2023sentiment, hasan2023zero}. The majority of the work in this domain involving LLMs is carried out in the English language \cite{rathje2023gpt, xing2024designing,zhang2023enhancing,zhang2023instruct}. Although Bangla is a low-resource language, there have been many studies carried out in sentiment analysis \cite{islam2021sentnob, hasan2020sentiment, hasan2023blp}. Unlike Bangla, there have been few studies done in Hindi \cite{patra2018sentiment} and Urdu \cite{muhammad2023innovations} languages. In contrast, for low-resource languages such as Bengali \cite{liu2023knowdee,hasan2023zero,kabir2023benllmeval}, Urdu \cite{koto2024zero}, and Hindi \cite{kumar2021sentiment, koto2024zero}, there has been a very limited number of works that use LLMs. Most of the work in these languages still primarily relies on language models and machine-learning approaches. 


%English
%Several works use instruction tuning and prompt engineering on LLM for sentiment analysis. \cite{sun2023sentiment} proposed a multi-LLM framework that overcomes the issues raised in a single LLM-based framework for sentiment analysis. In the sentiment analysis task of psychological data \cite{rathje2023gpt} used GPT 3.5 and 4 and showed LLM models produce nearly similar performance to machine learning models. 
%In terms of financial sentiment analysis researchers \cite{xing2024designing,zhang2023enhancing,zhang2023instruct} tend to avoid a direct approach instead they employ prompt or instruction tuning, for improving the predictive accuracy of LLM models
%Heterogeneous LLM Agents and Retrieval Augmented LLMs for improving the predictive accuracy of LLM models.
%Bengali
%Most sentiment analysis tasks in the Bengali language have been conducted using either statistical machine-learning algorithms or fine-tuned language models. There have been a few works recently that employ zero-shot and few-shot learning techniques on LLMs for Bengali sentiment analysis but fine-tuned language models have the edge over LLMs\cite{liu2023knowdee,goswami2023nlpbdpatriots,hasan2023zero,kabir2023benllmeval}. The performance of LLMs on Bengali sentiment analysis is not surprising as Bengali is a low-resource language. Despite not being outperformed by fine-tuned language models LLMs can be used to open a research horizon for low-resource language. LLMs can be utilized for sentiment analysis without developing a new dataset or training new models.  
%Urdu
%Hindi


%\subsection{Hatespeech Task}
%Hate speech detection is a challenging but important task aimed at identifying and mitigating offensive or harmful language in text data. Some of the commonly used techniques for detecting hate speech include machine learning \cite{abro2020automatic, mullah2021advances}, deep learning\cite{badjatiya2017deep,zimmerman2018improving}, transformer-based models\cite{mozafari2020hate,alatawi2021detecting}, and LLMs \cite{hee2024recent,garcia2023leveraging}. There has been a significant amount of work on hate speech, even in low-resource languages such as Bengali \cite{karim2021deephateexplainer,das2021bangla}, Urdu \cite{khan2021hate,ali2022hate} and Hindi \cite{santosh2019hate,vashistha2020online} However, most of these studies follow traditional machine learning or transformer-based models \cite{jahan2023systematic,chhabra2023literature}. Utilization of LLMs in the domain of hate speech detection could potentially be more beneficial for low-resource languages considering the scarcity of datasets\cite{hee2024recent,garcia2023leveraging}.  

==> sections/results_discussion.tex <==
\section{Results and Discussion}
\label{sec:result_discussion}
%This section presents the results and discussion of our experiments and findings.

%\subsection{Results}
%\label{ssec:result}
This section presents and discusses the performances of different LLMs for English vs low-resource languages. Further, we also discuss the performances of our experiments using different LLMs for different tasks in this section. Table \ref{tab:performance_nli}, Table \ref{tab:performance_senti}, and Table \ref{tab:performance_hate} represent the performances of NLI, sentiment, and hate speech tasks.


\subsection{English \textit{{vs}} Low-resource Languages}
%Compare Bangla, Hindi, and Urdu with English!

%LLMs are trained on hundreds of billions or trillions of tokens. The majority of the training data belongs to English languages due to the resource availability. 
In our study, our experiments show that all the LLMs consistently provide superior performances for English languages in all tasks except the performances of Gemini in the sentiment task. In the NLI task, the performance of GPT-4 in English is $18.04$\%, $17.38$\%, and $22.81$\% better than the Bangla, Hindi, and Urdu languages respectively (see Table \ref{tab:performance_nli}). Although Hindi performs better than Bangla and Urdu, there is still a massive performance gap compared to English. 
Besides, Llama 2 performance in English is $32.52$\%, $31.28$\%, and $29.94$\% higher compared with Bangla, Hindi, and Urdu respectively. The difference between English and other languages is $\sim$$70$\% from their original performance. Although the performance differences of Gemini between English and other languages are comparatively lower than GPT-4 and Llama 2, English is accomplishing approximately $13$\% better on average than Bangla, Hindi, and Urdu.


\begin{table}[!ht]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llrrrr}
\toprule
\multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Lang.}} & \multicolumn{1}{c}{\textbf{Acc.}} & \multicolumn{1}{c}{\textbf{P.}} & \multicolumn{1}{c}{\textbf{R.}} & \multicolumn{1}{c}{\textbf{F1$_{macro}$}}\\ \midrule

\multirow{4}{*}{\textbf{GPT-4}} & \textbf{EN} & 86.73 & 86.91 & 86.73 & \textbf{86.79} \\ \cline{2-6}
& \textbf{BN} & 68.73 & 75.95 & 68.73 & \textbf{68.75} \\ \cline{2-6}
& \textbf{HI} & 69.31 & 76.26 & 69.31 & \textbf{69.41} \\ \cline{2-6}
& \textbf{UR} & 64.52 & 72.90 & 64.52 & \textbf{63.98} \\ \midrule

\multirow{4}{*}{\textbf{Llama 2}} & \textbf{EN} & 74.47 & 76.27 & 74.47 & 74.82 \\ \cline{2-6}
& \textbf{BN} & 45.66 & 52.74 & 45.66 & 42.30 \\ \cline{2-6}
& \textbf{HI} & 47.29 & 65.68 & 47.29 & 43.54 \\ \cline{2-6}
& \textbf{UR} & 46.39 & 53.68 & 46.39 & 44.88 \\ \midrule

\multirow{4}{*}{\textbf{Gemini}} & \textbf{EN} & 78.40 & 78.06 & 78.40 & 78.12 \\ \cline{2-6}
& \textbf{BN} & 67.24 & 69.32 & 67.24 & 67.16 \\ \cline{2-6}
& \textbf{HI} & 66.48 & 68.67 & 66.48 & 66.50 \\ \cline{2-6}
& \textbf{UR} & 62.14 & 65.38 & 62.14 & 62.01 \\

\bottomrule
\end{tabular}
}
\caption{Performances of the NLI task across the models and languages. \textbf{Bold} indicates the best performances across the languages. Lang.: language, Acc.: accuracy, P.: Precision, R.: Recall, EN: English, BN: Bangla, HI: Hindi, and UR: Urdu}
\label{tab:performance_nli}
\end{table}

For the sentiment task, English is performing nearly on average $13\%$ better than other languages using GPT-4 (see Table~\ref{tab:performance_senti}). The performance difference of Llama 2 between English and other languages is $\sim11\%$ on average, and English is consistently doing better than other languages. Despite that, Bangla, Hindi, and Urdu are performing $0.49\%$, $0.89\%$, and $0.60\%$ better than English. The performance of Gemini remains almost the same for all the languages in the sentiment task.
Our hate speech task experiments reveal that the performance of GPT-4 in English is approximately, on average, $22\%$ better than low-resource languages (see Table \ref{tab:performance_hate}). Moreover, the performances in English are $\sim17\%$ and $\sim18\%$ better than low-resource languages for Llama 2 and Gemini models.

\begin{table}[!ht]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llrrrr}
\toprule
\multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Lang.}} & \multicolumn{1}{c}{\textbf{Acc.}} & \multicolumn{1}{c}{\textbf{P.}} & \multicolumn{1}{c}{\textbf{R.}} & \multicolumn{1}{c}{\textbf{F1$_{macro}$}}\\ \midrule

\multirow{4}{*}{\textbf{GPT-4}} & \textbf{EN} & 72.64 & 73.05 & 72.64 & \textbf{71.74} \\ \cline{2-6}
& \textbf{BN} & 61.33 & 64.57 & 61.33 & 56.36 \\ \cline{2-6}
& \textbf{HI} & 66.47 & 68.75 & 66.47 & 63.68 \\ \cline{2-6}
& \textbf{UR} & 62.31 & 64.89 & 62.31 & 58.19 \\ \midrule

\multirow{4}{*}{\textbf{Llama 2}} & \textbf{EN} & 55.64 & 66.89 & 55.64 & 53.38 \\ \cline{2-6}
& \textbf{BN} & 45.19 & 60.22 & 45.19 & 40.28 \\ \cline{2-6}
& \textbf{HI} & 48.31 & 63.32 & 48.31 & 43.73 \\ \cline{2-6}
& \textbf{UR} & 47.06 & 61.61 & 47.06 & 42.62 \\ \midrule

\multirow{4}{*}{\textbf{Gemini}} & \textbf{EN} & 64.59 & 67.86 & 64.59 & 64.44 \\ \cline{2-6}
& \textbf{BN} & 65.40 & 66.68 & 65.40 & \textbf{64.93} \\ \cline{2-6}
& \textbf{HI} & 65.87 & 67.14 & 65.87 & \textbf{65.33} \\ \cline{2-6}
& \textbf{UR} & 65.93 & 66.77 & 65.93 & \textbf{65.14} \\

\bottomrule
\end{tabular}
}
\caption{Performances of the Sentiment task across the models and languages. \textbf{Bold} indicates the best performances across the languages. Lang.: language, Acc.: accuracy, P.: Precision, R.: Recall, EN: English, BN: Bangla, HI: Hindi, and UR: Urdu}
\label{tab:performance_senti}
\end{table}


We postulate the low performance of LLMs in low-resource languages for the following reasons. One of the main reasons is that most of the LLMs are trained on a large amount of English data, i.e., $90\%$ of the training data of Llama 2 is English, whereas the amount of training data for low-resource languages is small compared with English. Moreover, cultural differences between English-spoken countries and low-resource language countries affect the sentiment and hate speech tasks the most. Lastly, the quality of the translation affects the performance of low-resource languages. However, Hindi performed better than Bangla and Urdu in all tasks among the low-resource languages. The performance difference among the low-resource languages is insignificant across the tasks and LLMs. Our findings from this section conclude that improving LLMs is required for low-resource languages.


%Although all the LLMs are showing excellent performances in resource-rich languages such as English in different tasks, there is much scope to improve the performance of LLMs for low-resource languages, i.e., Bangla, Urdu, etc. Among the low-resource languages, Hindi performed better than Bangla and Urdu in all tasks. The performance difference among the low-resource languages is not that significant across the tasks and LLMs. Our findings from this section conclude that the improvement of LLMs is required for low-resource languages.


\subsection{Comparison Among LLMs}
%How do LLMs perform?
We first analyzed the individual LLM outputs and found that GPT-4 could not predict much data on sentiment and hate speech tasks for Bangla and Urdu. Moreover, GPT-4 was able to provide predictions for all the English language samples for all the tasks. We also noticed that Llama 2 and Gemini models could predict all the samples from the NLI task for all languages. Llama 2 could not predict much data on the hate speech task for English. However, Llama 2 provides a small number of unpredicted data compared with GPT-4 for Bangla, Hindi, and Urdu. We analyzed the response of unpredicted data from GPT-4. We found that the model cannot understand the context to classify while Llama 2 could not predict due to inappropriate or offensive language. Moreover, the response from unpredicted samples from Llama includes repeated `l' only.
We briefly overview the unpredicted data in  Figure \ref{fig:unpredicted}. During the evaluation metrics calculation, we assigned the inverse classes for the unpredicted samples.


\begin{table}[!ht]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llrrrr}
\toprule
\multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Lang.}} & \multicolumn{1}{c}{\textbf{Acc.}} & \multicolumn{1}{c}{\textbf{P.}} & \multicolumn{1}{c}{\textbf{R.}} & \multicolumn{1}{c}{\textbf{F1$_{macro}$}}\\ \midrule

\multirow{4}{*}{\textbf{GPT-4}} & \textbf{EN} & 86.81 & 85.52 & 86.81 & \textbf{62.54} \\ \cline{2-6}
& \textbf{BN} & 55.32 & 75.51 & 55.32 & 38.79 \\ \cline{2-6}
& \textbf{HI} & 64.66 & 77.93 & 64.66 & \textbf{44.61} \\ \cline{2-6}
& \textbf{UR} & 54.00 & 75.18 & 54.00 & 38.66 \\ \midrule

\multirow{4}{*}{\textbf{Llama 2}} & \textbf{EN} & 79.32 & 83.93 & 79.32 & 60.04 \\ \cline{2-6}
& \textbf{BN} & 69.92 & 69.12 & 69.92 & \textbf{41.36} \\ \cline{2-6}
& \textbf{HI} & 74.54 & 71.58 & 74.54 & 44.39 \\ \cline{2-6}
& \textbf{UR} & 47.29 & 65.68 & 47.29 & \textbf{43.54} \\ \midrule

\multirow{4}{*}{\textbf{Gemini}} & \textbf{EN} & 58.00 & 77.69 & 58.00 & 49.10 \\ \cline{2-6}
& \textbf{BN} & 30.34 & 70.93 & 30.34 & 30.81 \\ \cline{2-6}
& \textbf{HI} & 32.01 & 72.72 & 32.01 & 33.36 \\ \cline{2-6}
& \textbf{UR} & 28.56 & 70.07 & 28.56 & 28.47 \\

\bottomrule
\end{tabular}
}
\caption{Performances of the Hate speech task across the models and languages. \textbf{Bold} indicates the best performances across the languages. Lang.: language, Acc.: accuracy, P.: Precision, R.: Recall, EN: English, BN: Bangla, HI: Hindi, and UR: Urdu}
\label{tab:performance_hate}
\end{table}

Gemini is the only LLM that predicted all the samples of each task. Although we provide a safety setting for the Gemini model, it blocked some data due to the content containing derogatory language. We noticed that the samples from sentiment and hate speech tasks were blocked for containing derogatory language, and those from the NLI task were not blocked. We provide a brief overview of the number of samples that are blocked by Gemini in Figure \ref{fig:blocked}. However, the Urdu language is not supported by the Gemini. Despite that, the Gemini performs strongly in Urdu for the NLI and sentiment tasks. We further investigated the performances of Gemini in the Urdu language. We found that the alphabets of Urdu are derived from the Arabic language family\footnote{\url{https://en.wikipedia.org/wiki/Urdu\_alphabet}} and many words are adopted from the Arabic language. Arabic is supported by Gemini, and the training data of Arabic shares semantic information with the Urdu language, which is why Gemini exhibits a strong performance in the Urdu language.


Further, we investigated the detailed performances of each task. GPT-4 shows superior performances on the NLI task for all languages while exhibiting good performances on the sentiment task. However, most hate class data were misclassified in the hate speech task for all languages. Llama 2 provides strong performances in English for NLI, sentiment, and hate speech tasks while finding difficulties in accurately predicting the contradiction, neutral, and hate classes for NLI, sentiment, and hate speech tasks, respectively. Although Llama 2 outperforms GPT-4 performances in hate class in every language, GPT-4 in English and Hindi is better than Llama 2 for hate speech tasks. Moreover, Llama 2 demonstrated comparatively better performance on the hate speech task than NLI and sentiment tasks. While Gemini exhibits strong performances in NLI and sentiment tasks for all the languages, it consistently performs poorly on the speech task for all the languages. However, Gemini performs comparatively better hate class performance than Llama 2 and GPT-4 for all the languages. Moreover, the performances in the neither and offensive classes are worse than other LLMs. We also found that most offensive classes are misclassified as neither. We provided the detailed class-wise experimental results in Appendix \ref{sec:appendix_b}.

In general, GPT-4 shows prominent performances over other LLMs across all the tasks. Although Llama 2 provides better results for hate speech tasks, it struggled to perform well in NLI and sentiment tasks. While Gemini demonstrated strong performances in NLI and sentiment tasks, it delivered worse in hate speech tasks. %Surprisingly, without prior training using Urdu data, Gemini exhibits outstanding performances in the Urdu language compared with others.



\subsection{Tasks Performances}
%\subsubsection{NLI Task}

\paragraph{NLI Task:}
We present the performances of different LLMs on the NLI task for English, Bangla, Hindi, and Urdu languages in Table \ref{tab:performance_nli}. GPT-4 exhibits superior performances for the NLI task with F1 scores of $86.79$, $68.75$, $69.41$, and $63.98$ in English, Bangla, Hindi, and Urdu, respectively. Llama2 provides F1 scores of $74.82$, $42.30$, $43.54$, and $44.88$ for English, Bangla, Hindi, and Urdu respectively. The F1 scores of Gemini are $78.12$, $67.16$, $66.50$, and $62.01$ in English, Bangla, Hindi, and Urdu, respectively. While Gemini outperforms Llama 2 in this task, GPT-4 outperforms in the NLI task.
%while Gemini delivers strong performances. However, Llama 2 shows moderate performances in Bangla, Hind, and Urdu for the NLI task while exhibiting comparative performance in the English language. 



%\subsubsection{Sentiment Task}

\paragraph{Sentiment Task:} Table \ref{tab:performance_senti} represents the performances of different LLMs on the sentiment task for English, Bangla, Hindi, and Urdu. With the use of GPT-4 zero-shot learning, we achieved F1 scores of $71.74$, $56.36$, $63.68$, and $58.19$ in English, Bangla, Hindi, and Urdu languages, respectively, while the F1 scores of Llama 2 zero-shot learning for the sentiment task are $53.38$, $40.28$, $43.73$, and $42.62$ in English, Bangla, Hindi, and Urdu. We obtained F1 scores of $64.44$, $64.93$, $65.33$, and $65.14$ for English, Bangla, Hindi, and Urdu. Gemini demonstrated superior performances in Bangla, Hindi, and Urdu, while GPT-4 outperformed in English for the sentiment task.


%\subsubsection{Hatespeech Task}

\paragraph{Hate Speech Task:}
We present the performances of the hate speech task using GPT-4, Gemini, and Llama 2 models for all languages in Table \ref{tab:performance_hate}. Using GPT-4 zero-shot learning, we achieved F1 scores of $62.54$, $38.79$, $44.61$, and $38.66$ in English, Bangla, Hindi, and Urdu respectively. F1 scores of $60.04$, $41.36$, $44.39$, and $43.54$ were achieved using Llama 2 in English, Bangla, Hindi, and Urdu, respectively. Moreover, the performance of GPT-4 is $0.22\%$ higher than Llama 2 in the Hindi language, which is comparable. Further, the performance of Gemini is relatively worse than GPT-4 and Llama2 with F1 scores of $49.10$, $30.81$, $33.36$, and $28.47$ in English, Bangla, Hindi, and Urdu languages respectively.

%GPT-4 outperforms the other LLMs in English and Hindi Languages while Llama 2 outperforms in Bangla and Urdu Languages. Moreover, the performance of GPT-4 is $0.22\%$ higher than Llama 2 in the Hindi language which is comparable. Besides, the performance of Gemini is not performing reasonably in comparison with GPT-4 and Llama 2.


%provide reasons for.
The overall performance of the NLI task is comparatively better than sentiment and hate speech tasks. The definition of an NLI task has clear rules and structured patterns, while sentiment and hate speech tasks are subjective and context-dependent. NLI task identifies the relation between two sentences based on structure and language logic \cite{bowman2015large} that makes the task easier for LLMs. Moreover, the context lies with the sentence pair, and LLMs can understand the context. While sentiment and hate speech tasks require understanding the tone of the text and sometimes the complex social and cultural contexts, these facts are challenging for LLMs to understand. 
Moreover, the data of the NLI task is incorporated from the well-structured MNLI corpus with precise labels and balanced classes, making the task more comfortable for LLMs. Unlike the NLI task, sentiment and hate speech task data are curated from social media platforms containing noise, informal expressions, slang, and incomplete text, making it challenging for LLMs. Moreover, most of the texts do not have the contexts within their representation, and it is challenging to identify the context for both humans and LLMs. Straightforward linguistics features and contextual information make the NLI task easier and perform better than sentiment and hate speech tasks using different LLMs.

%\todo[]{Need to write why NLI provides better results than sentiment and hatespeech}
%While GPT-4 and Gemini models show prominent performances on NLI and sentiment tasks, Llama 2 consistently exhibits poor performances in all the languages for the sentiment task and in Bangla, Hindi, and Urdu for the NLI task. Moreover, GPT-4 performances in Bangla for the sentiment task and in Urdu for both NLI and sentiment tasks are comparatively lower than the other languages. For the hatespeech task, the performances of the LLMs are not adequate for all the languages. The best system described in \cite{hateoffensive} on the hatespeech dataset reports an F1 score of 90\% while the F1 scores are 62.54 and 60.04 using GPT-4 and Llama 2 respectively in the English language. Moreover, the performances (considering F1 score) in other languages are below 45\%. In addition, Gemini consistently yields poor performances in all languages for the hatespeech task. 


%There are several challenges for developing resources in low-resource languages discussed in \cite{alam2021review}.

